23 DoF Grasping Policies from a Raw Point Cloud

Coordinating the motion of robots with high degrees of freedom (DoF) to grasp objects gives rise to many challenges. In this paper, we propose a novel imitation learning approach to learn a policy that directly predicts 23 DoF grasp trajectories from a partial point cloud provided by a single, fixed camera. At the core of the approach is a second-order geometric-based model of behavioral dynamics. This Neural Geometric Fabric (NGF) policy predicts accelerations directly in joint space. We show that our policy is capable of generalizing to novel objects, and combine our policy with a geometric fabric motion planner in a loop to generate stable grasping trajectories. We evaluate our approach on a set of three different objects, compare different policy structures, and run ablation studies to understand the importance of different object encodings for policy learning.

==> intro-fig.tex <==
\setcounter{figure}{1}
\makeatletter
\let\@oldmaketitle\@maketitle% Store \@maketitle
\renewcommand{\@maketitle}{\@oldmaketitle% Update \@maketitle to insert...
\begin{center}
  \centering
 \includegraphics[width=\textwidth]{images/intro_figure.png}
\end{center}
  %\refstepcounter{figure}
  \footnotesize{\textbf{Fig.~\thefigure:\label{fig:title}}~Our approach predicts 23 DoF trajectories based on raw point cloud and robot state (position and velocity) to grasp the object of interest. Some examples of resulting grasps are shown in top right. An example of a generated trajectory is shown in the bottom part of the figure. \vspace{-10pt}}
  \medskip}% ... an image
\makeatother
\shrinka
\maketitle
\shrinka

==> related-work.tex <==
A lot of work has been done to solve grasping. We split related work into two different categories depending on how grasping is achieved.

\textbf{Optimization} Papers in this category model grasping as an optimization problem and typically use a  gradient-based solver to solve it, but not always~\cite{ciocarlie-ijrr2009-eigengrasp, chen-2018-pSDF}. The metric to optimize over is either analytical~\cite{miller-icra99-force-wrench-space, ciocarlie-ijrr2009-eigengrasp, suarez-2009tro-contact-regions, suarez-2011ijrr-synthesizing-grasps, zheng-2005ijrr-force-closure-uncertainty, hang-tro2016-hierarchical-fingertip-space, siddiqui-frontiers2021-bayesian-exploration} or learned~\cite{lu-isrr2017-grasp-inference, lu-ral2019-grasp-type, lu-ram2020-MultiFingeredGP,lu-iros2020-active-grasp,vandermerwe-icra2020-reconstruction-grasping, matak-ral23-precision-grasps}. Typically, an IK optimization is necessary at some point in the optimization. Either when initializing the solution~\cite{vandermerwe-icra2020-reconstruction-grasping, matak-ral23-precision-grasps} or when converting the final solution to joint space~\cite{mousavian-iccv2019-graspnet}. Finally, another optimization is then necessary to compute the trajectory to get to the target solution. While these approaches are reliable and achieve remarkable success rates, they require solving several optimizations which can be time-consuming. 

\textbf{Imitation Learning}
As an alternative to optimization-based approaches, people have tried to learn a grasping policy. The policy predicts a solution to an optimization problem of interest without relying on a solver. This prediction would typically be a target robot configuration or a target end-effector pose. Such is a work from ~\cite{chen-implicit-shape-corl22}. They learn a policy that predicts a palm pose and hand configuration. Then, a manually derived arm controller is used to move the robot to the target configuration and a heuristic is used to close the fingers. In this work, we train a policy to predict the full trajectory in joint space directly.
The closest work to ours is by ~\cite{mandy-ngf-corl22}. In contrast to that work, we don't need human demonstrations but generate training data only in simulation. We don't need explicit object pose but ingest raw pointclouds. Finally, our approach works on a variety of objects, while~\cite{mandy-ngf-corl22} grasp only a single object.

These are submitted to icra: 
\cite{morel-grasp-trajectories-icra22} 
\cite{ye-continuous-grasp-function-arxiv22}

This is online
https://mimic-play.github.io/

\textbf{Reinforcement Learning}
Another way to train a grasping policy is reinforcement learning (RL). An example of such an approach is a framework presented by~\cite{osa-hierarchical-rl-grasping-iser2016}. They propose a two-level policy to grasp objects given a partial point cloud of an object. After determining potential grasp contact locations, the higher-level policy decides on the grasp location and grasp type. Then, the lower-level policy corresponding to the chosen grasp type executes the grasp.
